Nucleon Polarizabilities: from Compton Scattering to Hydrogen Atom

We review the current state of knowledge of the nucleon polarizabilities and of their role in nucleon Compton scattering and in hydrogen spectrum. We discuss the basic concepts, the recent lattice QCD calculations and advances in chiral effective-field theory. On the experimental side, we review the ongoing programs aimed to measure the nucleon (scalar and spin) polarizabilities via the Compton scattering processes, with real and virtual photons. A great part of the review is devoted to the general constraints based on unitarity, causality, discrete and continuous symmetries, which result in model-independent relations involving nucleon polarizabilities. We (re-)derive a variety of such relations and discuss their empirical value. The proton polarizability effects are presently the major sources of uncertainty in the assessment of the muonic hydrogen Lamb shift and hyperfine structure. Recent calculations of these effects are reviewed here in the context of the "proton-radius puzzle". We conclude with summary plots of the recent results and prospects for the near-future work.

==> sec8.tex <==
%\section{Conclusion and Outlook}
\section{Outlook}
\seclab{outlook}
In this section we examine the outlook for further progress in these areas of investigation, and outline some prospects for the near-future work. 
\begin{itemize}
\item Connection between VVCS
and VCS polarizabilities at finite $Q^2$:
\end{itemize}
